Model-checking an Epistemic \mu-calculus with Synchronous and Perfect Recall Semantics

We show that the model-checking problem is decidable for a fragment of the epistemic \mu-calculus. The fragment allows free variables within the scope of epistemic modalities in a restricted form that avoids constructing formulas embodying any form of common knowledge. Our calculus subsumes known decidable fragments of epistemic CTL/LTL. Its modal variant can express winning strategies in two-player games with one player having imperfect information and non-observable objectives, and, with a suitable encoding, decidable instances of the model-checking problem for ATL with imperfect information and perfect recall can be encoded as instances of the model-checking problem for this epistemic \mu-calculus.

==> exemplu.tex <==
%!TEX root = mu-calculus.tex

We exemplify the constructions above for the regular expression $R_2=\overline{a\overline{a}+aa}$. 
%The construction of $M_{R_2}$, we first consider the expression $R_0=a$. 
We start by associating with the expression $R_0 = a$ the first transition system in Figure \ref{fig:overview} 
with an empty set of agents, and the formula $\varphi_{R_0}=true$. 
Then, the expression $R_1=a\overline{a}+aa$ is associated with the MAS given by the union of the first two transition systems 
in Figure \ref{fig:overview} and an agent $A_{\Sigma''}$ which observes only $\Sigma''=\{a''\}$,
and the formula $\varphi_{R_1}=end_{\neg x}\vee K_{A_{\Sigma''}} \neg \varphi_1$. 
The expression $R_2$ is associated with the whole transition systems in Figure \ref{fig:overview} 
and the set of agents $\{A_{\Sigma'},A_{\Sigma''}\}$, where $A_{\Gamma'}$ observes only $\Sigma'=\{a'\}$,
and with the formula $\varphi_{R_2}=K_{A_{\Sigma'}} \neg \varphi_2$.
\begin{figure}[hbt]
\begin{tikzpicture}[->,bend angle=25,auto,node distance=.9cm] 
\tikzstyle{cvertex}=[minimum size=10pt,inner sep=0pt]
\tikzstyle{vertex}=[rectangle,thick,draw=black,minimum size=16pt,inner sep=1pt]
\tikzstyle{dvertex}=[rectangle,thick,draw=black,minimum size=12pt,inner sep=2pt]
{\scriptsize
\begin{scope}
\tikzset{node distance=1.3cm}
\node[vertex] (n1) [ ] { };
\node[vertex] (n2) [right of=n1] {$a''$};
\node[vertex] (n3) [right of=n2, node distance=1.3cm] {$end_{R_0}$};
\node[cvertex] (n4) [right of=n3,node distance=3.2cm]{$\varphi_1:\Diamond \Box end_{R_0}$};

\path (n1) edge[loop above] (n1); 
\path (n1) edge (n2);
\path (n2) edge (n3);
\path (n3) edge[loop above] (n3); 
\end{scope}

\begin{scope}[yshift=-1.5cm]
\tikzset{node distance=.9cm}
\node[vertex] (n1) [ ] { };
\node[vertex] (n2) [right of=n1] {$a'$};
\node[vertex] (n3) [right of=n2, node distance=1.3cm] {$a',a''$};
\node[vertex] (n4) [right of=n3, node distance=1.3cm] {$end_{R_1}$};
\node[vertex] (n5) [below of=n3, node distance=1.3cm] {$a'$};
\node[vertex] (n6) [right of=n5, node distance=1.8cm] {$end_{R_1},end_{x}$};
\node[cvertex] (n7) [right of=n4,node distance=3.2cm]{$\begin{array}{ll}\varphi_2:&\Diamond \Box (end_{R_1}\land \\[.5mm] &(end_{\neg x}\vee K_{A_{\Gamma''}} \neg \varphi_1))\end{array}$};

\path (n1) edge[loop above] (n1); 
\path (n1) edge (n2);
\path (n2) edge (n3);
\path (n3) edge[loop above] (n3); 
\path (n3) edge (n4);
\path (n2) edge (n5);
\path (n5) edge (n6);
\path (n6) edge[loop below] (n6); 
\end{scope}

\begin{scope}[yshift=-4cm]
\tikzset{node distance=1.3cm}
\node[vertex] (n1) [] {$a,a'$};
\node[vertex] (n2) [right of=n1, node distance=1.3cm] {$end_{R_2}$};
\node[cvertex] (n3) [right of=n2,node distance=5.4cm]{$\varphi_3:\Diamond \Box (end_{R_2}\land K_{A_{\Gamma'}} \neg \varphi_2)$};

\path (n1) edge[loop above] (n1); 
\path (n1) edge (n2);
\path (n2) edge[loop above] (n2); 
\end{scope}
}
\end{tikzpicture}
\caption{Reducing the emptiness of $\overline{a\overline{a}+aa}$ to the model checking problem for the \munonmix}
\label{fig:overview}
\vspace{-5mm}
\end{figure}

==> lowerBound.tex <==
%!TEX root = mu-calculus.tex

\def\cM{\mathcal{M}}
\def\cR{\mathcal{R}}

\section{The complexity of the model checking problem for the \munonmix}

This section is devoted to the proof of the following result.
We will use here the CTL$^*$ operator $E \Diamond \Box$, 
expressible in \muknl as 
$E\Diamond \Box \phi = \mu Z_1.(\nu Z_2.(\phi \land EX Z_2) \vee EX Z_1)$.

\begin{theorem}
The model checking problem for the \munonmix is hard for non-elementary time.
\end{theorem}
\begin{proof}
The lower bound is showed using a reduction from the emptiness problem for star-free regular languages. 
We denote $\br E$ the complementation of the expression $E$.
%Let $\Sigma$ be a finite alphabet. 
%Star-free regular languages are described by regular expressions constructed from the letters in $\Sigma$, 
%the empty set symbol $\emptyset$, the boolean operators union $\cup$, intersection $\cap$, 
%and complementation $\overline{\phantom{r}}$, and the concatenation operator $\cdot$. 


We may define the set of \emph{context star-free expressions} as the least set of expressions built as follows:
\begin{itemize}
\item Any star-free expression without complementation is a context star-free expression.
\item If $C(x_1,\ldots,x_n)$ is a star-free, complementation-free expression over $\Sigma\cup\{x_1,\ldots,x_n\}$ 
%not employing the complementation operator 
in which each $x_i$ appears exactly once 
and $F_1$,$\ldots$,$F_n$ are context star-free expressions, then $C(\overline{F_1},\ldots,\overline{F_n})$ 
obtained from $C$ by replacing $x_i$ with $\overline{F_i}$, for all $1\leq i\leq n$, belongs to $\cR$.

An extra restriction that we impose to the expressions $F_i$ is that $\eps \not \in L(F_i)$.
\end{itemize}
It is easy to see that any star-free expression over $\Sigma$
is a context star-free expression.

%An extra restriction that we impose on our context star-free expressions is 
%that 

We prove that for any context star-free expression $R$ over $\Sigma$, there exists a 
multi-agent system \\
$M_R=\big(Q,Ag,\delta,q_0,\Pi,(\Pi_a)_{a\in Ag},\pi\big)$, where 
$\Sigma\subseteq \bigcup_{a\in Ag}\Pi_a$, an atomic proposition 
$end_R$ not in $\Sigma$ 
and a \muknl formula $\varphi_R$ such that
\begin{align}
w\in L(R) \mbox{ iff }& \text{there exists a path $\rho$ in $M_R$ with }\rho\restr{\Sigma} = w\notag\\
& \text{ and which satisfies } \Diamond \Box (end_R\land \varphi_R) 
\label{eq_red}
%&& \mbox{of its labeling on $\Sigma$ is exactly $w$}
\end{align}
%\end{array}
%\end{equation}
%Recall that $\rho\restr{\Sigma}$ stands for the sequence of 
%$\Sigma$-labels of states in the run $\rho$.
Property (\ref{eq_red}) implies $L(R) \neq \emptyset$ iff $M_R\models  E\, \Diamond \Box (end_R\land \varphi_R)$.


%Above, $\Diamond$ and $\Box$ denote the ``eventually'' and the ``always'' operator from the temporal logic CTL$^*$, respectively. 
%Clearly, this implies that $L(R)$ is non-empty iff $M_R\models  E\, \Diamond \Box (end_R\land \varphi_R)$, 
%where $E$ is the existential quantification over paths from CTL$^*$. %E \Diamond 


%The formula $E\, \Diamond \Box (end_R\land \varphi_R)$ can be written in $\mu$-calculus as:
%\vspace{-2mm}
%\[
%\mu Z_1.(\nu Z_2.(end_R\land \varphi_R'\land EX Z_2) \vee EX Z_1),
%\vspace{-2mm}
%\]
%where $\varphi_R'$ is the $\mu$-calculus formula equivalent to $\varphi_R$.

We proceed by structural induction. 
For the base case, let $R$ be a regular expression without complementation over some alphabet $\Sigma$. 
Build a finite Moore (i.e. state-labeled) automaton $A = (Q, \delta, q_0,Q_F,\Sigma,\pi)$, where $\pi:Q\sd\Sigma$ and
$Q_F$ is the set of final states, such that $L(A) = L(R)$, then transform it into a MAS with no agents
$
M_R=\big(Q_R,\emptyset,\delta_R,q_0,\Pi_R,\emptyset,\pi_R\big),
$
where $Q_R = Q \cup \{q_f^R\}$, $\Pi_R = \Pi \cup\{end_R\}$,
$\pi_R\restr{\Pi} = \pi$, $\pi_R(q_f^R) = \{end_R\}$,
and 
$\delta_R = \delta\cup \{q_f^R\sd q_f^R\} \cup \{q\sd q_f^R \mid q \in Q_f\}$.
Also put $\varphi_R=true$. Clearly, property (\ref{eq_red}) holds.

%in which states are labeled by symbols in $\Sigma\cup\{end\}$ 
%where the set of states and the transition relation are defined as in the finite automaton 
%(where states are labeled by alphabet symbols) that accepts the language $L(R)$ 
%except that (1) every accepting state is connected to a distinguished state labeled 
%by $end_R$ which has a self loop and (2) every other state is connected to a distinguished unlabeled state which also has a self loop. 
%labeled also by $end_R$ and it is

For the induction step, we prove in detail only the case of unary contexts,
the case of multiple contexts being treated similarly.
So let $C(x)$ be a star-free expression without complementation 
over $\Sigma\cup\{x\}$ in which the symbol $x$ appears exactly once and 
$F$ a context star-free expression over $\Sigma$. 
%W.l.o.g. we suppose that $(\Sigma\cup\{x\})\cap\Gamma=\emptyset$. 
%We prove that property (\ref{eq_red}) holds for $R=C(\overline{F})$. 
%The general case that considers regular expressions of the form $C(\overline{F_1},\ldots,\overline{F_n})$ is similar.

By the induction hypothesis, there exists a 
MAS $M_F=\big(Q_1,Ag_1,\delta_1,Q_0^1,\Pi_1,(\Pi^1_a)_{a\in Ag_1},\pi_1\big)$ with 
$\Pi \supseteq\Sigma$, an atom $end_F\in \Pi \setminus \Sigma$, and a formula $\varphi_F$ 
satisfying the property (\ref{eq_red}).

%$w\in L(F)$ iff  $M_F$ contains a path satisfying $\Diamond \Box (end_F\land \varphi_F)$
%whose labeling projected on $\Gamma$ is $w$.

We  build a finite automaton $A_{C(x)} = (Q_2,\delta_2,Q_0^2,Q_f^2,\Sigma\cup\{x\},\pi_2)$
equivalent with $C(x)$.
W.l.o.g. we may assume that there exists a single state $q_x \in Q$ labeled with $x$, 
and that $Q_f$ is partitioned as $Q_f = Q_f^x \cup Q_f^{\neg x}$, 
with $Q_f^{\neg x}$ denoting the final states which can be reached without passing through $q_x$, and 
$Q_f^{x} = Q_f\setminus Q_f^{\neg x}$.

Consider also a copy $\Sigma'$ of $\Sigma$, and denote $Diag(\Sigma,\Sigma') = \{(a,a') \mid a \in \Sigma\}$.
The MAS for $C(\br F)$ is then the union of a modification of $M_F$ and 
a modification of $A_{C(x)}$. 
The modification of $M_F$ appends a new initial looping state $\br q_0$ without labels
and replaces all symbols from $\Sigma$ with their copies in $\Sigma'$.
The modification of $A_{C(x)}$ turns it into a larger automaton 
by replacing the state $q_x$ with a Moore automaton accepting $Diag(\Sigma,\Sigma')^*$;
we also append two new looping states $q_{end_{\neg x}}$ and $q_{end_{x}}$ 
which are only reached from $Q_f^{\neg x}$, resp. from $Q_f^x$, and are labeled with $end_{C(\br F)}$, resp. $end_x$ and $end_{C(\br F)}$.
In the new MAS, there will be a new agent $A_{\Sigma'}$ which 
observes only the symbols in $\Sigma'$.

Formally, we get the MAS
$M_{C(\br F)} = \big(Q,Ag,\delta,Q_0,\Pi,(\Pi_a)_{a\in Ag},\pi\big)$ with
$Q = Q_1\cup Q_2\cup \br\Sigma\cup \{\br q_0,q_{end_x},q_{end_{\neg x}}\}$,
$Q_0 = Q_0^2 \cup \{\br q_0\}$.
$\Pi = \Pi_1 \cup \Sigma'\cup \{end_x,end_{C(\br F)}\}$ and $Ag = Ag_1 \cup \{A_{\Sigma'}\}$.
$\Pi_a^1 = \Pi_a$ for all $a \in Ag_1$, $\Pi_{A_{\Sigma'}} = \Sigma'$.
$\pi(q_1) = \{ a' \mid a \in \pi_1(q_1)\}$ for all $q_1 \in Q_1$, 
$\pi(q_2) = \pi_2(q_2)$ for all $q_2\in Q_2\setminus \{q_x\}$,
$\pi(\br a) = \{a,a'\}$ for all $a \in \br\Sigma$,
$\pi(q_{end_x}) = \{end_x,end_{C(\br F)}\}$, $\pi(end_{\neg x}) = \{end_{C(\br F)}\}$, $\pi(\br q_0) = \emptyset$.
$\delta$ is defined as follows:
%contains all transitions in $\delta_1$ and in $\delta_2$ that do not enter $q_x$, plus the following sets of transitions:
\begin{align*}
\delta & = \delta_1 \cup \big( \delta_2 \setminus \{ q\sd q_x,q_x \sd q \mid q \in Q_2\} \big) \\
& \cup \big\{ \br a \sd \br b, q\sd\br a, \br a\sd r \mid a,b \in \Sigma, q\sd q_x, q_x \sd r \in \delta \big\} \\
& \cup \big\{ q \sd q_{end_x} \mid q \in Q_f^x \big\}  \cup \big\{ q \sd q_{end_{\neg x}}  \mid q \in Q_f^{\neg x} \big\} \\
& \cup \big\{ \br q_0 \sd \br q_0, \br q_0 \sd q_0 \mid q_0 \in Q_0^1 \big\} \\
& \cup \{  q_{end_x} \sd  q_{end_x}, q_{end_{\neg x}} \sd q_{end_{\neg x}} \big\}
\end{align*}
Also put
$
%\varphi_{E(\overline{F})}= \Box \big((\bigvee_{p\in\Gamma} p\land X \bigwedge_{p\in\Gamma}\neg p)\Rightarrow (X K_{A_{\overline{F}}}\,\neg\,(end_F\land \varphi_F))\big)
\varphi_{C(\overline{F})}=end_{x}\sd K_{A_{\Sigma'}}\Box \Diamond \neg (end_F\land \varphi_F)
$.


%Formally, $A_{C(*)} = (Q^*,\delta^*,Q_0, \{q_{end_x},q_{end_{\neg x}}\},\Sigma\cup Diag(\Sigma,\Sigma')\cup \{


%First, we construct a multi-agent system
%\[
%M_{C(x)}=\big(Q^1,\emptyset,\delta^1,q_0^1,\Sigma\cup\{x,end_{C(\overline{F})},end_{\neg x}\},\emptyset,\pi^1\big)
%\]
%for the regular expression $C(x)$ similar to the base case. 
%First, $Q^1$ and $\delta^1$ include the set of states and the transition relation 
%of a finite automaton that accepts the language $L(C(x))$ such that any path that 
%goes through a state labeled by $x$ is disjoint from a path that does not go through such a state. 
%Then, (1) every accepting state $q$ of the finite automaton such that all the paths 
%from the initial state $q_0^1$ to $q$ don't go through a state labeled by $x$ 
%are connected to a distinguished state labeled by $end_{C(\overline{F})}$ 
%and $end_{\neg x}$ which has a self loop, (2) every other accepting state 
%is connected to a distinguished state labeled by $end_{C(\overline{F})}$ 
%which has a self loop, and (3) every other state is connected to a distinguished 
%unlabeled state which also has a self loop. 


%in which states are labeled by symbols in $\Sigma\cup\{x,end\}$ such that every path ending in a state labeled by the fresh atomic proposition $end\not\in\Sigma\cup\Gamma$ corresponds to a word in $L(E(x))$. 
%
%Notice that because the regular expression does not contain Kleene star the transition system $M_{E(x)}$ does not contain cycles. We modify $M_{E(x)}$ as follows: 
%\begin{itemize}
%	\item the label $a\in\Sigma\cup\{x\}$ of every predecessor of a state labeled by $x$ is replaced with $(a,\$)$,
%	\item the label $a\in\Sigma\cup\{x\}$ of every successor of a state labeled by $x$ is replaced with $(a,\#)$, and 
%	\item every state labeled by $x$ is replaced by an automaton with labeled states representing the language $\Gamma^*$. 
%\end{itemize}

%Second, let $M_F'$ be the multi-agent system obtained from $M_F$ by 
%(1) substituting every symbol $\alpha\in\Gamma$ with a new symbol $\alpha'$ and 
%(2) adding an unlabeled state with a self-loop which is connected to the initial state. 
%Let $\Gamma'$ denote the set of new symbols. Also, let $M_{C(*)}$ be the multi-agent system 
%obtained from $M_{C(x)}$ by replacing every state labeled by $x$ with an automaton 
%with labeled states representing the language $\{(\alpha,\alpha')\mid \alpha\in \Gamma\}^*$ 
%and by adding a new agent $A_{\Gamma'}$ which observes only atomic propositions from $\Gamma'$. 

%Third, let $M_{C(\overline{F})}$ be the union between $M_{C(*)}$ and the multi-agent system $M_F'$. 
%The union is defined as usual by adding an initial state which is connected to the initial 
%states of the two MAS, by taking the union of the sets of states, of the transition relations, of the set of atomic propositions, and of the set of agents. 

%Then, we define
%\[
%M_{C(\overline{F})}=(M_{C(\overline{F})},Ag\cup \{A_{\overline{F}}\},(\Pi_a\mid a\in Ag\cup \{A_{\overline{F}}\})),
%\] 
%where $\Pi_{A_{\overline{F}}}=\Gamma$, and 


To prove that property (\ref{eq_red}) holds for $R=C(\overline{F})$, 
%\[
%\begin{array}{lcl}
%w\in L(E(\overline{F}))&\mbox{ iff }& \cM_{E(\overline{F})}\mbox{ contains a path satisfying } \\[1mm]
%&&\Diamond \Box (end_{E(\overline{F})}\land \varphi_{E(\overline{F})}) \mbox{such that}\\[1mm]
%&&\mbox{the projection of its labeling on $\Sigma\cup\Gamma$ is $w$}.
%\end{array}
%\]
take $w \in L(C(\overline{F}))$. 
%By the construction of $M_{C(*)}$ 
Clearly, there exists a path $\rho$ in $M_{C(F)}$  with $\rho \restr{\Sigma} = w$
and ending either in $q_{end_x}$ or in $q_{end_{\neg x}}$. 
If $\rho$ ends in $q_{end_{\neg x}}$, then, by construction of $M_{C(\br F)}$, $\rho$
never passes through states in $\br \Sigma$, and, therefore, 
there exists no run $\rho'$ that passes through states in $Q_1$ with $\rho \sim_{A_{\Sigma'}} \rho'$.
In conclusion, $\rho$ satisfies $\Box \Diamond K_{A_{\Sigma'}}\neg end_F$,
and therefore satisfies 
$\Box \Diamond K_{A_{\Sigma'}}\neg (end_F\land \varphi_F)$.

%Consequently, $\pi$ satisfies $\Diamond end$.
Suppose now $\rho$ does not end in $q_{end_{\neg x}}$.
% and, therefore,  
%Because $w\in L(C(\overline{F}))$,
%and, similarly, 
It then follows that 
$w=w_1\cdot w_2\cdot w_3$ with 
$w_2\in L(\overline{F})$ and $w_1xw_3 \in C(x)$.
Let $w_2'$ be the word obtained from $w_2$ by substituting every symbol in $\Sigma$ with its copy in $\Sigma'$.
Note first that, by the induction hypothesis, %$w_2'\in L(\overline{F})$ implies that 
any path $\rho'$ in 
$M_F$ with $\rho'\restr{\Sigma} = w_2$ satisfies
$\Box \Diamond \neg ( end_F\land \varphi_F)$.
%, where $\varphi'_F$ is obtained from $\varphi_F$ by renaming 
%all symbols from $\Sigma$ into their copies in $\Sigma'$.
%That is, the run $\rho'$ cannot end in a state labeled $end_F$.

Take then any run $\rho''$ with $\rho'' \sim_{A_{\Sigma'}} \rho$.
It must be decomposable as
$\rho'' = \rho_1''\cdot \rho_2'' \cdot \rho_3''$ with $\rho_2''\restr{\Sigma'} = w_2'$.
So either $\rho''$ ends in $q_{end_{\neg x}}$, or it is a run in $Q_1 \cup \{\br q_0\}$. If it ends in $q_{end_{\neg x}}$ then 
it satisfies $\Box \Diamond K_{A_{\Sigma'}}\neg end_F$. Otherwise, 
if we remove from $\rho''$ all the initial loops in $\br q_0$,  
replace all symbols in $\Sigma'$ with their copies in $\Sigma$, and 
denote the resulting suffix $\br \rho$, we obtain a run in $M_F$ with $\br\rho\restr{\Sigma} = w_2$.
As we observed above, this means that $\br\rho$ does not satisfy $\Diamond \Box (end_F\land \varphi_F)$
%end in a state labeled $end_F$,
a property which must also hold for $\rho''$.
In conclusion, %all $\rho''\sim_{A_{C(\br F)}} \rho$ satisfy 
$\rho$ satisfies $\Box \Diamond K_{A_{C(\br F)}}\neg (end_F\land \varphi_F)$.

%which only occur when passing through the states in $\br \Sigma$.
%Therefore, $\rho''\restr{\Sigma'} = w_2'$ and 
%all the 



%By the definition of $M_F'$, $w_2\in L(\overline{F})$ implies that any path in $M_F'$ 
%whose labeling projected on $\Gamma'$ is $w_2'$ satisfies $\Box \Diamond \neg ( end_F\land \varphi_F)$.
%the same holds for the transition system obtained from $M_F$ by adding a loop over an unlabeled state before its initial state. 

%Let $\rho'$ be a prefix of $\rho$ ending in $end_{C(\overline{F})}$. 
%If this state is also labeled by $end_{\neg x}$ then $\pi$ satisfies 
%$\Box \Diamond (end_{C(\overline{F})}\land \varphi_{C(\overline{F})})$. 
%Otherwise, let $\pi''$ be a path in $M_{C(\overline{F})}$ containing a prefix of length 
%$|\pi'|$ that has the same observation w.r.t the agent $A_{\Gamma'}$ as the path $\pi'$. 
%If this path belongs to $M_{C(*)}$ then it satisfies $\Box\Diamond \neg (end_F\land \varphi_F)$ 
%because there exists no state in $M_{C(*)}$ labeled by $end_F$. 
%If $\pi''$ belongs to $M_F'$ then, 
%%and $\pi''$ a path in $M_F'$ containing a prefix of length $|\pi'|$ that has the same observation w.r.t the agent $A_{\Gamma'}$ as the path $\pi'$. 
%because $A_{\Gamma'}$ can observe all the symbols in $\Gamma'$, the projection of the labeling 
%of $\pi''$ on $\Gamma'$ is exactly $w_2'$. 
%Consequently, it satisfies $\Box \Diamond \neg ( end_F\land \varphi_F)$ 
%and the last state of $\pi'$ satisfies $\varphi_{C(\overline{F})}$. 

Now, let $\rho$ be a run in $M_{C(\overline{F})}$ which satisfies 
$\Diamond\Box (end_{C(\overline{F})}\land \varphi_{C(\overline{F})})$. 
By construction, this run 
%belongs to $M_{C(\Gamma^*)}$ and it 
ends in a loop 
over a state labeled by $end_{C(\overline{F})}$. 
If this state is not labeled by $end_x$ then the projection of the labeling 
of $\rho$ on $\Sigma$ is clearly in $L(C(\overline{F}))$. 
Otherwise, its labeling projected on $\Sigma$ is of the form 
$w=w_1\cdot w_2\cdot w_3$, where $w_2\in L(\overline{F})$ and $w_1xw_3 \in C(x)$.
%$w_1$, $w_2$, and $w_3$ are as above. 
We have to prove that $w_2\not\in L(F)$. 
Because the run $\rho$ satisfies $\varphi_{C(\overline{F})}$, 
we obtain that any run $\rho'$ that passes only through states in $Q_1$ and 
whose projection on $\Sigma'$ is $w_2'$ 
satisfies $\Box \Diamond \neg (end_F\land \varphi_F)$. 
By the induction hypothesis and the construction of $M_F$, the latter implies $w_2\not\in L(F)$.
\end{proof}

\input{exemplu.tex}



